Parallel Louvain Community Detection Optimized for GPUs

Community detection now is an important operation in numerous graph based applications. It is used to reveal groups that exist within real world networks without imposing prior size or cardinality constraints on the set of communities. Despite its potential, the support for parallel computers is rather limited. The cause is largely the irregularity of the algorithm and the underlying heuristics imply a sequential nature. In this paper a GPU based parallelized version of the Louvain method is presented. The Louvain method is a multi-phase, iterative heuristic for modularity optimization. It was originally developed by Blondel et al. (2008), the method has become increasingly popular owing to its ability to detect high modularity community partitions in a fast and memory-efficient manner. The parallel heuristics used, were first introduced by Hao Lu et al. (2015). As the Louvain method is inherently sequential, it limits the possibility of scalable usage. Thanks to the proposed parallel heuristics, I observe how this method can behave on GPUs. For evaluation I implemented the heuristics using CUDA on a GeForce GTX 980 GPU and for testing Ive used organization landscapes from the CERN developed Collaboration Spotting project that involves patents and publications to visualize the connections in technologies among its collaborators. Compared to the parallel Louvain implementation running on 8 threads on the same machine that has the used GPU, the CUDA implementation is able to produce community outputs comparable to the CPU generated results, while providing absolute speedups of up to 30 using the GeForce GTX 980 consumer grade GPU.

==> mybibfile.tex <==
@article{findcom,
  title   = "Finding and evaluating community structure in networks",
  journal = "Phys. Rev. E",
  volume  = "69",
  year    = "2004",
  doi     = "026113",
  author  = "M.E.J. Newman and M. Girvan"
}

@article{comdet,
  title   = "Community detection in graphs",
  journal = "Phys. Rep.",
  volume  = "486",
  pages   = "75-–174",
  year    = "2010",
  doi     = "10.1016/j.physrep.2009.11.002",
  author  = "S. Fortunato"
}

@article{rescom,
  title   = "Narrow scope for resolution-limit-free community detection",
  journal = "Phys. Rev. E",
  volume  = "1",
  year    = "2011",
  doi     = "016114",
  author  = "V.A. Traag, P. Van Dooren and Y. Nesterov"
}

@article{modgraph,
  title   = "Modularity and graph algorithms",
  journal = "SIAM AN10 Minisymposium on Analyzing Massive Real-World Graphs",
  pages = "12--16"
  year    = "2009",,
  author  = "D. Bader and J. McCloskey"
}

@article{comdetres,
  title   = "Community detection in graphs",
  journal = "Phys. Rev. E",
  volume  = "83",
  year    = "2011",
  doi     = "056119",
  author  = "J.W. Berry, B. Hendrickson, R.A. LaViolette and C.A. Phillips"
}

@article{louvainalg,
  title   = "Fast unfolding of communities in large networks",
  journal = "Journal of Statistical Mechanics: Theory and Experiment",
  volume  = "10",
  year    = "2008",
  doi     = "P10008",
  author  = "Vincent D Blondel, Jean-Loup Guillaume, Renaud Lambiotte and Etienne Lefebvre"
}

@article{clustering,
  title   = "On modularity clustering",
  journal = "IEEE Trans. Knowl. Data Eng.",
  volume = "20",
  pages = "172--188"
  year    = "2008",
  author  = "U. Brandes, D. Delling, M. Gaertler, R. Gorke, M. Hoefer, Z. Nikoloski and D. Wagner"
}

@article{graphpart,
  title   = "Graph partitioning models for parallel computing",
  journal = "Parallel Comput.",
  volume = "26",
  pages = "1519-–1534"
  year    = "2000",
  author  = "B. Hendrickson and T.G. Kolda"
}

@article{parlouvain,
  title   = "Parallel heuristics for scalable community detection",
  journal = "Parallel Computing",
  volume = "47",
  pages = "1937"
  year    = "2015",
  author  = "Hao Lu, Mahantesh Halappanavar and Ananth Kalyanaraman"
}
 
@article{cudaposter,
  title   = "Yang-Mills on CUDA",
  journal = "GPU Technology Conference",
  year    = "2013",
  author  = "R. Forster and A. Fulop"
}

@article{cudaarticle,
  title   = "Yang-Mills on CUDA",
  journal = "Acta Univ. Sapientiae, Informatica",
  year    = "2013",
  author  = "R. Forster, A. Fulop"
}

@article{cudaarticle2,
  title   = "Chaotic behavior of the lattice Yang-Mills on CUDA",
  journal = "Acta Univ. Sapientiae, Informatica",
  volume = "7",
  pages = "216-−238",
  year    = "2013",
  author  = "R. Forster, A. Fulop"
}

@article{cuda,
  title   = "CUDA C Programming Guide",
  year    = "2015",
  author  = "NVIDIA Corp."
}

@article{fermi,
  title   = "Whitepaper NVIDIA's Next Generation Compute Architecture: Fermi",
  year    = "2009",
  author  = "NVIDIA Corp."
}

@article{msc,
  title   = "Scheduling of Parallel Algorithms on CUDA Capable GPUs Masters Thesis",
  year    = "2015",
  author  = "R. Forster"
}

@article{bh,
  title   = "Programming Massively Parallel Processors: A Hands-on Approach",
  journal = "Acta Univ. Sapientiae, Informatica",
  year    = "2012",
  author  = "David B. Kirk, Wen-mei W. Hwu"
} 

@article{ines,
  title   = "Louvain Community Detection with Parallel Heuristics On GPUs",
  journal = "20th Jubilee IEEE International Conference on Intelligent Engineering Systems",
  volume = "20",
  pages = "227--233",
  year    = "2016",
  author  = "R. Forster"
}

